Speaking at the Right Level: Literacy-Controlled Counterspeech Generation with RAG-RL

Health misinformation spreading online poses a significant threat to public health. Researchers have explored methods for automatically generating counterspeech to health misinformation as a mitigation strategy. Existing approaches often produce uniform responses, ignoring that the health literacy level of the audience could affect the accessibility and effectiveness of counterspeech. We propose a Controlled-Literacy framework using retrieval-augmented generation (RAG) with reinforcement learning (RL) to generate tailored counterspeech adapted to different health literacy levels. In particular, we retrieve knowledge aligned with specific health literacy levels, enabling accessible and factual information to support generation. We design a reward function incorporating subjective user preferences and objective readability-based rewards to optimize counterspeech to the target health literacy level. Experiment results show that Controlled-Literacy outperforms baselines by generating more accessible and user-preferred counterspeech. This research contributes to more equitable and impactful public health communication by improving the accessibility and comprehension of counterspeech to health misinformation

==> latex/table_tex/main-results.tex <==

\begin{table*}[bth!
]
\centering
\small

\begin{tabular}{lllccc}
\toprule
\textbf{Model} & \textbf{Method} & \textbf{Literacy Level} & \textbf{Politeness} & \textbf{Target Distance (↓)} & \textbf{Effectiveness} \\
\midrule

\multirow{12}{*}{LLaMA} 
& \multirow{4}{*}{Direct Prompt} 
    & Low    & 0.51 (0.20) & 16.64 & 0.73 (0.12) \\
&   & Medium & 0.62 (0.24) & 12.94 & 0.73 (0.07) \\
&   & High   & 0.36 (0.22) & 0.00  & 0.75 (0.03) \\
&   & \textbf{Avg.} & 0.50 & 9.86 & 0.74 \\
\cmidrule(l){2-6}

& \multirow{4}{*}{Prompt Engineering} 
    & Low    & 0.39 (0.23) & 0.00 & 0.75 (0.03) \\
&   & Medium & 0.49 (0.22) & 1.07 & 0.74 (0.06) \\
&   & High   & 0.35 (0.19) & 0.00 & 0.75 (0.04) \\
&   & \textbf{Avg.} & 0.41 & 0.36 & \textbf{0.75} \\
\cmidrule(l){2-6}

& \multirow{4}{*}{RAG (Separate KB)} 
    & Low    & 0.72 (0.25) & 0.00 & 0.71 (0.13) \\
&   & Medium & 0.66 (0.22) & 0.00 & 0.71 (0.13) \\
&   & High   & 0.41 (0.21) & 0.00 & 0.72 (0.09) \\
&   & \textbf{Avg.} & 0.60 & 0.00 & 0.71 \\
\cmidrule(l){2-6}

& \multirow{4}{*}{RAG GRPO (55 FKRE + Effect)} 
    & Low    & 0.84 (0.15) & 0.00 & 0.74 (0.07) \\
&   & Medium & 0.69 (0.20) & 0.00 & 0.73 (0.10) \\
&   & High   & 0.98 (0.02) & 0.00 & 0.75 (0.00) \\
&   & \cellcolor{gray!20}\textbf{Avg.} & \cellcolor{gray!20}\textbf{0.84} & \cellcolor{gray!20}\textbf{0.00} & \cellcolor{gray!20}0.74 \\
\midrule

\multirow{12}{*}{Qwen} 
& \multirow{4}{*}{Direct Prompt} 
    & Low    & 0.65 (0.28) & 0.00 & 0.75 (0.05) \\
&   & Medium & 0.65 (0.26) & 4.87 & 0.75 (0.02) \\
&   & High   & 0.37 (0.22) & 0.00 & 0.75 (0.00) \\
&   & \textbf{Avg.} & 0.56 & 1.62 & \textbf{0.75} \\
\cmidrule(l){2-6}

& \multirow{4}{*}{Prompt Engineering} 
    & Low    & 0.36 (0.22) & 0.00 & 0.74 (0.06) \\
&   & Medium & 0.48 (0.23) & 0.00 & 0.73 (0.13) \\
&   & High   & 0.41 (0.18) & 0.00 & 0.73 (0.12) \\
&   & \textbf{Avg.} & 0.42 & 0.00 & 0.73 \\
\cmidrule(l){2-6}

& \multirow{4}{*}{RAG (Separate KB)} 
    & Low    & 0.69 (0.25) & 0.00 & 0.69 (0.16) \\
&   & Medium & 0.52 (0.18) & 0.00 & 0.68 (0.18) \\
&   & High   & 0.45 (0.19) & 0.00 & 0.73 (0.07) \\
&   & \textbf{Avg.} & 0.55 & 0.00 & 0.70 \\
\cmidrule(l){2-6}

& \multirow{4}{*}{RAG GRPO (55 FKRE + Effect)} 
    & Low    & 0.77 (0.18) & 0.00 & 0.73 (0.11) \\
&   & Medium & 0.55 (0.19) & 0.00 & 0.74 (0.08) \\
&   & High   & 0.86 (0.22) & 0.00 & 0.75 (0.04) \\
% \rowcolor{gray!15}
&   & \cellcolor{gray!20}\textbf{Avg.} & \cellcolor{gray!20}\textbf{0.73} & \cellcolor{gray!20}\textbf{0.00} & \cellcolor{gray!20}0.74 \\
\midrule

\multirow{12}{*}{Mistral} 
& \multirow{4}{*}{Direct Prompt} 
    & Low    & 0.20 (0.19) & 0.00 & 0.71 (0.11) \\
&   & Medium & 0.37 (0.23) & 3.45 & 0.75 (0.02) \\
&   & High   & 0.33 (0.21) & 0.00 & 0.75 (0.02) \\
&   & \textbf{Avg.} & 0.30 & 1.15 & 0.74 \\
\cmidrule(l){2-6}

& \multirow{4}{*}{Prompt Engineering} 
    & Low    & 0.27 (0.22) & 0.00 & 0.74 (0.06) \\
&   & Medium & 0.31 (0.20) & 0.00 & 0.72 (0.15) \\
&   & High   & 0.40 (0.23) & 0.00 & 0.75 (0.02) \\
&   & \textbf{Avg.} & 0.29 & 0.00 & 0.74 \\
\cmidrule(l){2-6}

& \multirow{4}{*}{RAG (Separate KB)} 
    & Low    & 0.37 (0.23) & 0.00 & 0.69 (0.16) \\
&   & Medium & 0.40 (0.22) & 0.00 & 0.71 (0.13) \\
&   & High   & 0.43 (0.21) & 0.00 & 0.74 (0.05) \\
&   & \textbf{Avg.} & 0.40 & 0.00 & 0.71 \\
\cmidrule(l){2-6}

& \multirow{4}{*}{RAG GRPO (55 FKRE + Effect)} 
    & Low    & 0.88 (0.10) & 0.00 & 0.69 (0.15) \\
&   & Medium & 0.70 (0.21) & 0.00 & 0.70 (0.15) \\
&   & High   & 0.97 (0.07) & 0.00 & 0.74 (0.04) \\
&   & \textbf{Avg.} & \textbf{0.85} & 0.00 & 0.71 \\

\bottomrule
\end{tabular}
\caption{Comparative Performance Across Models, Methods, and Literacy Levels}
\end{table*}

==> latex/table_tex/new_prompt_baseline1.tex <==
\begin{table*}[htbp]
\centering
\begin{tabular}{llcccc}
\toprule
\textbf{Method} & \textbf{Literacy Level} & \textbf{Politeness} & \textbf{Readability} & \textbf{Target Distance} & \textbf{Effectiveness} \\
\midrule
\multirow{4}{*}{Direct Prompt}
 & low    & 0.51 (0.20) & 63.60 (9.77) & 16.64 & 0.73 (0.12) \\
 & medium & 0.62 (0.24) & 47.06 (9.67) & 12.94 & 0.73 (0.07) \\
 & high   & 0.36 (0.22) & 35.31 (9.99) & 0.00  & 0.75 (0.03) \\
 \cdashline{2-6} 
 & Average& 0.50        & --          & 9.86  & 0.74        \\
\midrule
\multirow{4}{*}{Prompt Engineering}
 & low    & 0.39 (0.23) & 81.40 (6.92) & 0.00  & 0.75 (0.03) \\
 & medium & 0.49 (0.22) & 58.93 (13.13)& 1.07  & 0.74 (0.06) \\
 & high   & 0.35 (0.19) & 36.47 (9.82) & 0.00  & 0.75 (0.04) \\
 \cdashline{2-6} 
 & Average& 0.41        & --           & 0.36  & 0.75        \\
\bottomrule
\end{tabular}
\caption{Performance comparison of two baseline methods across literacy levels. Values are mean (standard deviation).}
\label{tab:direct_vs_prompt}
\end{table*}


==> latex/table_tex/new_prompt_baseline_rag.tex <==

\begin{table*}[htbp]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{llcccc}
\toprule
\textbf{Method} & \textbf{Literacy Level} & \textbf{Politeness} & \textbf{Readability} & \textbf{Target Distance} & \textbf{Effectiveness} \\
\midrule

\multirow{4}{*}{Direct Prompt}
 & low    & 0.51 (0.20) & 63.60 (9.77) & 16.64 & 0.73 (0.12) \\
 & medium & 0.62 (0.24) & 47.06 (9.67) & 12.94 & 0.73 (0.07) \\
 & high   & 0.36 (0.22) & 35.31 (9.99) & 0.00  & 0.75 (0.03) \\
 \cdashline{2-6} 
 & Average& 0.50        & --          & 9.86  & 0.74        \\
\midrule
\multirow{4}{*}{Prompt Engineering}
 & low    & 0.39 (0.23) & 81.40 (6.92) & 0.00  & 0.75 (0.03) \\
 & medium & 0.49 (0.22) & 58.93 (13.13)& 1.07  & 0.74 (0.06) \\
 & high   & 0.35 (0.19) & 36.47 (9.82) & 0.00  & 0.75 (0.04) \\
 \cdashline{2-6} 
 & Average& 0.41        & --           & 0.36  & 0.75        \\
 \midrule

% \multirow{4}{*}{RAG w/ Combined KB} 
%   & low    & 0.49 (0.23) & 79.48 (11.59) & 0.52 & 0.70 (0.16) \\
%   & medium & 0.54 (0.22) & 61.95 (12.59) & 0.00 & 0.73 (0.10) \\
%   & high   & 0.40 (0.21) & 40.74 (14.14) & 0.00 & 0.73 (0.08) \\
%    \cdashline{2-6} 
%   & Average& 0.48        & --            & 0.17 & 0.72        \\

% \midrule
% \multirow{4}{*}{RAG w/ Combined KB + Web Search}
%   & low    & 0.50 (0.27) & 81.73 (7.41)  & 0.00 & 0.74 (0.05) \\
%   & medium & 0.53 (0.23) & 63.39 (12.91) & 0.00 & 0.73 (0.09) \\
%   & high   & 0.38 (0.19) & 39.63 (10.13) & 0.00 & 0.74 (0.05) \\
%    \cdashline{2-6} 
%   & Average& 0.47        & --            & 0.00 & 0.74        \\

% \midrule
% \multirow{4}{*}{RAG + Web Search + Summarized Evidence}
%   & low    & 0.49 (0.26) & 78.76 (7.63)  & 1.24 & 0.73 (0.09) \\
%   & medium & 0.54 (0.26) & 60.88 (13.73) & 0.00 & 0.71 (0.11) \\
%   & high   & 0.37 (0.18) & 36.58 (9.80)  & 0.00 & 0.74 (0.05) \\
%    \cdashline{2-6} 
%   & Average& 0.47        & --            & 0.41 & 0.73        \\

% \midrule
\multirow{4}{*}{Tailored RAG (Separate KB)} 
  & low    & 0.53 (0.23) & 83.69 (10.87) & 0.00 & 0.60 (0.26) \\
  & medium & 0.64 (0.21) & 64.96 (13.94) & 0.00 & 0.56 (0.29) \\
  & high   & 0.44 (0.25) & 41.22 (11.37) & 0.00 & 0.75 (0.04) \\
   \cdashline{2-6} 
  & Average& 0.54        & --            & 0.00 & 0.64        \\

\midrule
\multirow{4}{*}{Tailored RAG + Web Search}
  & low    & 0.56 (0.28) & 81.96 (8.07)  & 0.00 & 0.74 (0.06) \\
  & medium & 0.56 (0.24) & 65.61 (12.72) & 0.00 & 0.73 (0.08) \\
  & high   & 0.39 (0.19) & 39.08 (10.45) & 0.00 & 0.74 (0.05) \\
\cdashline{2-6} 

  & Average& 0.50        & --            & 0.00 & 0.74        \\

 \midrule
\multirow{4}{*}{RAG + Tailored KB +  GRPO only FKRE}
 & low    & 0.68 (0.22) & 84.58 (6.40) &	0.00 &	0.75 (0.02) \\
 & medium & 0.59 (0.19) & 74.29 (9.59) &	0.00 &	0.69 (0.19) \\
 & high   & 0.56 (0.31) & 33.60 (8.45) &	0.00 &	0.74 (0.08) \\
 \cdashline{2-6}
 & Average& 0.61        & --           & 0.00 & 0.73        \\

%  \midrule
% \multirow{4}{*}{RAG + Tailored KB +  GRPO only Effectiveness}

% \midrule
% \multirow{4}{*}{RAG + Tailored KB +  GRPO only FKRE}

% \midrule
% \multirow{4}{*}{RAG + Tailored KB +  GRPO  FKRE + Effecetiveness+ politeness}
 

\bottomrule
\end{tabular}
}
\caption{Performance of RAG-based methods across health literacy levels. Values are reported as mean (standard deviation).}
\label{tab:rag_methods_comparison}
\end{table*}




==> latex/table_tex/new_prompt_finetune.tex <==
\begin{table*}[htbp]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{llcccc}
\toprule
\textbf{Method} & \textbf{Literacy Level} & \textbf{Politeness} & \textbf{Readability} & \textbf{Target Distance} & \textbf{Effectiveness} \\
\midrule

\multirow{4}{*}{Finetuned LLM}
 & low    & 0.82 (0.15) & 80.39 (5.71) & 0.00 & 0.75 (0.02) \\
 & medium & 0.63 (0.22) & 63.21 (8.74) & 0.00 & 0.75 (0.00) \\
 & high   & 0.97 (0.03) & 34.51 (7.36) & 0.00 & 0.75 (0.01) \\
 \cdashline{2-6}
 & Average& 0.81        & --           & 0.00 & 0.75        \\


% \midrule
% \multirow{4}{*}{Finetuned LLM + PPO Optimization}
%  & low    & 0.83 (0.15) & 80.52 (6.18) & 0.00 & 0.75 (0.00) \\
%  & medium & 0.65 (0.23) & 63.50 (9.15) & 0.00 & 0.75 (0.00) \\
%  & high   & 0.97 (0.05) & 35.44 (8.22) & 0.00 & 0.75 (0.00) \\
%  \cdashline{2-6}
%  & Average& \textbf{0.82}       & --           & \textbf{0.00} & \textbf{0.75}        \\

\midrule
\multirow{4}{*}{Finetuned LLM + GRPO Optimization only FKRE}
 & low    & 0.83 (0.14) & 79.89 (5.32) & 0.11 & 0.74 (0.06) \\
 & medium & 0.61 (0.21) & 65.83 (8.56) & 0.00 & 0.75 (0.03) \\
 & high   & 0.96 (0.08) & 34.94 (7.68) & 0.00 & 0.75 (0.00) \\
 \cdashline{2-6}
 & Average& 0.80        & --           & 0.04 & 0.75        \\


\midrule
\multirow{4}{*}{Finetuned LLM + GRPO Optimization  FKRE \& effectiveness (6:4)}
 & low    & 0.81 (0.16) & 80.50 (5.29) & 0.00 & 0.75 (0.00) \\
 & medium & 0.65 (0.24) & 64.68 (11.03) & 0.00 & 0.72 (0.14) \\
 & high   & 0.48 (0.25) & 32.87 (9.38) &	0.00 &	0.75 (0.03) \\
 \cdashline{2-6}
 & Average& 0.65        & --           & 0.00 & 0.74        \\

\midrule
\multirow{4}{*}{Finetuned LLM + GRPO Optimization  FKRE \& effectiveness (5:5)}
 & low    & 0.84 (0.13) & 80.28 (5.29) &	0.00 &	0.75 (0.00) \\
 & medium & 0.62 (0.21) & 66.43 (9.35) &	0.00 &	0.75 (0.00) \\
 & high   & 0.96 (0.08) & 35.22 (7.77) &	0.00 &	0.75 (0.00) \\
 \cdashline{2-6}
 & Average& 0.81        & --           & 0.00 & 0.75        \\

\midrule
\multirow{4}{*}{Finetuned LLM + GRPO Optimization  FKRE \& effectiveness \& politeness (5:3:2)}
 & low    & 0.80 (0.15) & 80.97 (5.77) &	0.00 &	0.75 (0.00) \\
 & medium & 0.63 (0.21) & 66.73 (9.01) &	0.00 &	0.75 (0.00) \\
 & high   & 0.97 (0.05) & 34.10 (7.70) &	0.00 &	0.75 (0.00) \\
 \cdashline{2-6}
 & Average& 0.80        & --           & 0.00 & 0.75        \\

\midrule
\multirow{4}{*}{Tailored RAG (Separate KB)} 
  & low    & 0.53 (0.23) & 83.69 (10.87) & 0.00 & 0.60 (0.26) \\
  & medium & 0.64 (0.21) & 64.96 (13.94) & 0.00 & 0.56 (0.29) \\
  & high   & 0.44 (0.25) & 41.22 (11.37) & 0.00 & 0.75 (0.04) \\
   \cdashline{2-6} 
  & Average& 0.54        & --            & 0.00 & 0.64        \\


\midrule
\multirow{4}{*}{RAG + Tailored KB + Finetuned LLM}
 & low    & 0.68 (0.20) & 85.06 (6.89) & 0.00 & 0.74 (0.06) \\
 & medium & 0.55 (0.19) & 72.32 (11.52)& 0.00 & 0.68 (0.19) \\
 & high   & 0.54 (0.30) & 32.40 (12.23)& 0.00 & 0.73 (0.10) \\
 \cdashline{2-6}
 & Average& 0.59        & --           & 0.00 & 0.72        \\


\midrule
\multirow{4}{*}{RAG + Tailored KB +  GRPO only FKRE}
 & low    & 0.68 (0.22) & 84.58 (6.40) &	0.00 &	0.75 (0.02) \\
 & medium & 0.59 (0.19) & 74.29 (9.59) &	0.00 &	0.69 (0.19) \\
 & high   & 0.56 (0.31) & 33.60 (8.45) &	0.00 &	0.74 (0.08) \\
 \cdashline{2-6}
 & Average& 0.61        & --           & 0.00 & 0.73        \\


\midrule
\multirow{4}{*}{RAG + Tailored KB +  GRPO FKRE \& effectiveness (6:4)}
 & low    & 0.65 (0.22) & 85.13 (6.60) &	0.00 &	0.75 (0.00) \\
 & medium & 0.56 (0.20) & 74.21 (13.30) & 0.00 &	0.62 (0.25) \\
 & high   & 0.58 (0.31) & 38.35 (29.88) & 0.00 &	0.73 (0.13) \\
 \cdashline{2-6}
 & Average& 0.60        & --           & 0.00 & 0.70        \\

 
\bottomrule
\end{tabular}
}
\caption{Performance of finetuned LLMs with or without GRPO optimization across health literacy levels. Values are mean (standard deviation).}
\label{tab:finetune_rl_comparison}
\end{table*}


==> latex/table_tex/prompt_wo_tag.tex <==
\begin{table*}[htbp]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{llcccc}
\toprule
                                Method & Literacy Level &  Politeness &   Readability & Target Distance & Effectiveness \\
\midrule
                         Direct Prompt &            low & 0.51 (0.20) &  63.60 (9.77) &           16.64 &   0.73 (0.12) \\
                                       &         medium & 0.62 (0.24) &  47.06 (9.67) &           12.94 &   0.73 (0.07) \\
                                       &           high & 0.36 (0.22) &  35.31 (9.99) &            0.00 &   0.75 (0.03) \\
                                        \cdashline{2-6}
                                       &        Average &        0.50 &            -- &            9.86 &          0.74 \\
                                       \midrule
                    Prompt Engineering &            low & 0.61 (0.28) &  70.36 (9.45) &            9.64 &   0.74 (0.04) \\
                                       &         medium & 0.66 (0.29) & 50.34 (11.03) &            9.66 &   0.73 (0.06) \\
                                       &           high & 0.35 (0.21) & 36.92 (10.04) &            0.00 &   0.75 (0.03) \\
                                        \cdashline{2-6}
                                       &        Average &        0.54 &            -- &            6.43 &          0.74 \\
                                       \midrule
                    RAG w/ Combined KB &            low & 0.53 (0.24) & 67.69 (11.98) &           12.31 &   0.68 (0.16) \\
                                       &         medium & 0.74 (0.24) & 49.87 (10.34) &           10.13 &   0.66 (0.18) \\
                                       &           high & 0.65 (0.28) & 39.63 (10.51) &            0.00 &   0.71 (0.13) \\
                                        \cdashline{2-6}
                                       &        Average &        0.64 &            -- &            7.48 &          0.68 \\
                                       \midrule
       RAG w/ Combined KB + Web Search &            low & 0.43 (0.25) & 72.12 (10.06) &            7.88 &   0.72 (0.09) \\
                                       &         medium & 0.63 (0.30) & 48.80 (11.41) &            11.2 &   0.68 (0.13) \\
                                       &           high & 0.46 (0.26) & 38.31 (10.71) &            0.00 &   0.73 (0.07) \\
                                        \cdashline{2-6}
                                       &        Average &        0.51 &            -- &            6.36 &          0.71 \\
                                       \midrule
RAG + Web Search + Summarized Evidence &            low & 0.64 (0.26) &  70.09 (9.81) &            9.91 &   0.71 (0.11) \\
                                       &         medium & 0.77 (0.20) &  47.63 (9.82) &           12.37 &   0.64 (0.16) \\
                                       &           high & 0.73 (0.22) &  38.57 (8.88) &            0.00 &   0.73 (0.07) \\
                                        \cdashline{2-6}
                                       &        Average &        0.71 &            -- &            7.43 &          0.69 \\
                                       \midrule
                          Tailored RAG &            low & 0.65 (0.23) & 75.38 (12.33) &            4.62 &   0.52 (0.25) \\
                                       &         medium & 0.82 (0.20) & 56.25 (11.00) &            3.75 &   0.58 (0.27) \\
                                       &           high & 0.71 (0.26) & 37.37 (10.14) &            0.00 &   0.68 (0.16) \\
                                        \cdashline{2-6}
                                       &        Average &        0.73 &            -- &            \textbf{2.79} &          0.59 \\
                                       \midrule
                         Finetuned LLM &            low & 0.92 (0.14) &  69.62 (7.75) &           10.38 &   0.75 (0.01) \\
                                       &         medium & 0.95 (0.12) &  45.19 (9.54) &           14.81 &   0.75 (0.02) \\
                                       &           high & 0.98 (0.01) &  27.77 (7.92) &            0.00 &   0.75 (0.01) \\
                                        \cdashline{2-6}
                                       &        Average &        0.95 &            -- &            8.40 &          0.75 \\
           %                             \midrule
           % Finetuned LLM + PPO  &            low & 0.94 (0.09) &  67.99 (6.77) &           12.01 &   0.75 (0.00) \\
           %                             &         medium & 0.92 (0.17) &  47.54 (9.07) &           12.46 &   0.75 (0.03) \\
           %                             &           high & 0.98 (0.01) &  29.08 (8.20) &            0.00 &   0.74 (0.05) \\
           %                              \cdashline{2-6}
           %                             &        Average &        \textbf{0.95} &            -- &            8.16 &          \textbf{0.75} \\
\bottomrule
\end{tabular}
}
\caption{Performance of different methods across health literacy levels when using prompts without a target tag. Values are mean (standard deviation).}
\label{tab:finetune_rl_comparison}
\end{table*}



==> latex/table_tex/training_data.tex <==
\begin{table*}[htbp]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{llcccc}
\toprule
\textbf{Method} & \textbf{Literacy Level} & \textbf{Politeness} & \textbf{Readability} & \textbf{Target Distance} & \textbf{Effectiveness} \\
\midrule

\multirow{4}{*}{\parbox{5.5cm}{\centering Check\_COVID\_GPT-4o-mini \\ (w/o target FKRE tag)}}
 & low    & 0.94 (0.08) & 70.59 (6.64) & 9.41  & 0.75 (0.00) \\
 & medium & 0.97 (0.09) & 46.70 (8.71) & 13.30 & 0.75 (0.00) \\
 & high   & 0.98 (0.04) & 23.35 (7.99) & 0.00  & 0.75 (0.01) \\
  \cdashline{2-6}
 & Average& 0.96        & \textemdash  & 7.57  & 0.75        \\

\addlinespace
\midrule

\multirow{4}{*}{\parbox{5.5cm}{\centering Check\_COVID\_GPT-4o-mini \\ (with FKRE tag)}}
 & low    & 0.84 (0.13) & 80.02 (5.76) & 0.00  & 0.75 (0.00) \\
 & medium & 0.79 (0.16) & 64.58 (7.63) & 0.00  & 0.75 (0.01) \\
 & high   & 0.82 (0.22) & 28.68 (8.51) & 0.00  & 0.75 (0.00) \\
  \cdashline{2-6}
 & Average& 0.82        & \textemdash  & \textbf{0.00}  & \textbf{0.75}        \\

\bottomrule
\end{tabular}
}
\caption{Performance of GPT-4o-mini (1006 samples) before and after prompt revision with FKRE targets. Values are shown as mean (standard deviation).}
\label{tab:gpt4o_fkrt_revision}
\end{table*}


==> latex/table_tex_main/Check_Covid.tex <==
\begin{table*}[htb!]
\centering
\small
\renewcommand{\arraystretch}{0.9}
\begin{tabular}{llccc}
\toprule
\textbf{Method} & \textbf{Literacy Level} & \textbf{Politeness} & \textbf{Target Distance (↓)} & \textbf{User Preference} \\
\midrule

\multicolumn{5}{l}{\textbf{LLaMA-8B}} \\
Direct Prompt        
    & low     & 0.53 (0.22) & 11.98 & 0.63 (0.25) \\
    & medium  & 0.70 (0.18) & 13.44 & 0.72 (0.09) \\
    & high    & 0.54 (0.15) & 0.00  & 0.74 (0.05) \\
    & \textbf{Avg.} & \textbf{0.59} & \textbf{8.47} & \textbf{0.70} \\
% \cmidrule(l){1-5}
Prompt Engineering   
    & low     & 0.52 (0.19) & 0.00  & 0.74 (0.06) \\
    & medium  & 0.60 (0.17) & 0.21  & 0.74 (0.08) \\
    & high    & 0.51 (0.12) & 0.00  & 0.74 (0.07) \\
    & \textbf{Avg.} & \textbf{0.54} & \textbf{0.07} & \textbf{0.74} \\
% \cmidrule(l){1-5}
RAG       
    & low     & 0.72 (0.19) & 0.00  & 0.74 (0.06) \\
    & medium  & 0.74 (0.16) & 0.00  & 0.74 (0.07) \\
    & high    & 0.57 (0.13) & 0.00  & 0.70 (0.11) \\
    & \textbf{Avg.} & \textbf{0.68} & \textbf{0.00} & \textbf{0.73} \\
% \cmidrule(l){1-5}
\textbf{\textit{Controlled-Literacy}}
% Controlled-Literacy 
    & low     & 0.82 (0.12) & 0.00  & 0.75 (0.00) \\
    & medium  & 0.75 (0.15) & 0.00  & 0.75 (0.02) \\
    & high    & 0.99 (0.00) & 0.00  & 0.75 (0.02) \\
    & \cellcolor{gray!20}\textbf{Avg.} & \cellcolor{gray!20}\textbf{0.85} & \cellcolor{gray!20}\textbf{0.00} & \cellcolor{gray!20}\textbf{0.75} \\

\midrule
\multicolumn{5}{l}{\textbf{LLaMA-1B}} \\
Direct Prompt       
    & low     & 0.59 (0.27) & 15.32 & 0.52 (0.24) \\
    & medium  & 0.67 (0.22) & 8.36  & 0.51 (0.20) \\
    & high    & 0.52 (0.21) & 0.00  & 0.62 (0.17) \\
    & \textbf{Avg.} & \textbf{0.59} & \textbf{7.89} & \textbf{0.55} \\
% \cmidrule(l){1-5}
Prompt Engineering   
    & low     & 0.68 (0.21) & 1.43  & 0.65 (0.19) \\
    & medium  & 0.50 (0.19) & 16.56 & 0.55 (0.23) \\
    & high    & 0.84 (0.17) & 0.00  & 0.65 (0.16) \\
    & \textbf{Avg.} & \textbf{0.67} & \textbf{6.00} & \textbf{0.62} \\
% \cmidrule(l){1-5}
RAG         
    & low     & 0.52 (0.19) & 15.93 & 0.41 (0.24) \\
    & medium  & 0.55 (0.15) & 5.37  & 0.43 (0.23) \\
    & high    & 0.57 (0.17) & 0.00  & 0.43 (0.21) \\
    & \textbf{Avg.} & \textbf{0.55} & \textbf{7.10} & \textbf{0.42} \\
% \cmidrule(l){1-5}
\textbf{\textit{Controlled-Literacy}}
% Controlled-Literacy 
    & low     & 0.80 (0.14) & 0.00  & 0.71 (0.13) \\
    & medium  & 0.79 (0.17) & 0.00  & 0.72 (0.10) \\
    & high    & 0.83 (0.27) & 0.00  & 0.68 (0.13) \\
    & \cellcolor{gray!20}\textbf{Avg.} & \cellcolor{gray!20}\textbf{0.81} & \cellcolor{gray!20}\textbf{0.00} & \cellcolor{gray!20}\textbf{0.70} \\

\midrule
\multicolumn{5}{l}{\textbf{Qwen-7B}} \\
Direct Prompt       
    & low     & 0.74 (0.24) & 0.00  & 0.76 (0.08) \\
    & medium  & 0.64 (0.21) & 1.58  & 0.75 (0.04) \\
    & high    & 0.52 (0.15) & 0.00  & 0.75 (0.01) \\
    & \textbf{Avg.} & \textbf{0.63} & \textbf{0.53} & \textbf{0.75} \\
% \cmidrule(l){1-5}
Prompt Engineering   
    & low     & 0.46 (0.18) & 1.58  & 0.73 (0.10) \\
    & medium  & 0.59 (0.18) & 0.00  & 0.74 (0.11) \\
    & high    & 0.53 (0.13) & 0.00  & 0.74 (0.10) \\
    & \textbf{Avg.} & \textbf{0.53} & \textbf{0.53} & \textbf{0.74} \\
% \cmidrule(l){1-5}
RAG         
    & low     & 0.58 (0.17) & 2.38  & 0.74 (0.07) \\
    & medium  & 0.64 (0.16) & 3.38  & 0.75 (0.04) \\
    & high    & 0.63 (0.14) & 0.00  & 0.73 (0.08) \\
    & \textbf{Avg.} & \textbf{0.62} & \textbf{0.00} & \textbf{0.74} \\
% \cmidrule(l){1-5}
\textbf{\textit{Controlled-Literacy}}
% Controlled-Literacy  
    & low     & 0.79 (0.16) & 0.00  & 0.75 (0.04) \\
    & medium  & 0.62 (0.13) & 0.00  & 0.75 (0.04) \\
    & high    & 0.88 (0.18) & 0.00  & 0.74 (0.05) \\
    & \cellcolor{gray!20}\textbf{Avg.} & \cellcolor{gray!20}\textbf{0.76} & \cellcolor{gray!20}\textbf{0.00} & \cellcolor{gray!20}\textbf{0.75} \\

\bottomrule
\end{tabular}
\caption{Cross generalization performance on \textbf{CheckCovid Dataset}. The best overall performance in each category is highlighted in gray.}
\label{tab:checkcovid_results}
\end{table*}


==> latex/table_tex_main/Check_Covid_best.tex <==
\begin{table*}[htb!]
\centering
\small
\renewcommand{\arraystretch}{0.9}
\begin{tabular}{llccc}
\toprule
\textbf{Method} & \textbf{Literacy Level} & \textbf{Politeness} & \textbf{Target Distance (↓)} & \textbf{User Preference} \\
\midrule

\multicolumn{5}{l}{\textbf{LLaMA-8B}} \\
Direct Prompt        
    & low     & 0.53 (0.22) & 11.98 & 0.63 (0.25) \\
    & medium  & 0.70 (0.18) & 13.44 & 0.72 (0.09) \\
    & high    & 0.54 (0.15) & 0.00  & 0.74 (0.05) \\
    & \textbf{Avg.} & \textbf{0.59} & \textbf{8.47} & \textbf{0.70} \\
% \cmidrule(l){1-5}
Prompt Engineering   
    & low     & 0.52 (0.19) & 0.00  & 0.74 (0.06) \\
    & medium  & 0.60 (0.17) & 0.21  & 0.74 (0.08) \\
    & high    & 0.51 (0.12) & 0.00  & 0.74 (0.07) \\
    & \textbf{Avg.} & \textbf{0.54} & \textbf{0.07} & \textbf{0.74} \\
% \cmidrule(l){1-5}
RAG       
    & low     & 0.72 (0.19) & 0.00  & 0.74 (0.06) \\
    & medium  & 0.74 (0.16) & 0.00  & 0.74 (0.07) \\
    & high    & 0.57 (0.13) & 0.00  & 0.70 (0.11) \\
    & \textbf{Avg.} & \textbf{0.68} & \textbf{0.00} & \textbf{0.73} \\
% \cmidrule(l){1-5}
\textbf{\textit{Controlled-Literacy}}
% Controlled-Literacy 
    & low     & 0.82 (0.12) & 0.00  & 0.75 (0.00) \\
    & medium  & 0.75 (0.15) & 0.00  & 0.75 (0.02) \\
    & high    & 0.99 (0.00) & 0.00  & 0.75 (0.02) \\
    & \cellcolor{gray!20}\textbf{Avg.} & \cellcolor{gray!20}\textbf{0.85} & \cellcolor{gray!20}\textbf{0.00} & \cellcolor{gray!20}\textbf{0.75} \\

% \midrule
% \multicolumn{5}{l}{\textbf{LLaMA-1B}} \\
% Direct Prompt       
%     & low     & 0.59 (0.27) & 15.32 & 0.52 (0.24) \\
%     & medium  & 0.67 (0.22) & 8.36  & 0.51 (0.20) \\
%     & high    & 0.52 (0.21) & 0.00  & 0.62 (0.17) \\
%     & \textbf{Avg.} & \textbf{0.59} & \textbf{7.89} & \textbf{0.55} \\
% % \cmidrule(l){1-5}
% Prompt Engineering   
%     & low     & 0.68 (0.21) & 1.43  & 0.65 (0.19) \\
%     & medium  & 0.50 (0.19) & 16.56 & 0.55 (0.23) \\
%     & high    & 0.84 (0.17) & 0.00  & 0.65 (0.16) \\
%     & \textbf{Avg.} & \textbf{0.67} & \textbf{6.00} & \textbf{0.62} \\
% % \cmidrule(l){1-5}
% RAG         
%     & low     & 0.52 (0.19) & 15.93 & 0.41 (0.24) \\
%     & medium  & 0.55 (0.15) & 5.37  & 0.43 (0.23) \\
%     & high    & 0.57 (0.17) & 0.00  & 0.43 (0.21) \\
%     & \textbf{Avg.} & \textbf{0.55} & \textbf{7.10} & \textbf{0.42} \\
% % \cmidrule(l){1-5}
% \textbf{\textit{Controlled-Literacy}}
% % Controlled-Literacy 
%     & low     & 0.80 (0.14) & 0.00  & 0.71 (0.13) \\
%     & medium  & 0.79 (0.17) & 0.00  & 0.72 (0.10) \\
%     & high    & 0.83 (0.27) & 0.00  & 0.68 (0.13) \\
%     & \cellcolor{gray!20}\textbf{Avg.} & \cellcolor{gray!20}\textbf{0.81} & \cellcolor{gray!20}\textbf{0.00} & \cellcolor{gray!20}\textbf{0.70} \\

% \midrule
% \multicolumn{5}{l}{\textbf{Qwen-7B}} \\
% Direct Prompt       
%     & low     & 0.74 (0.24) & 0.00  & 0.76 (0.08) \\
%     & medium  & 0.64 (0.21) & 1.58  & 0.75 (0.04) \\
%     & high    & 0.52 (0.15) & 0.00  & 0.75 (0.01) \\
%     & \textbf{Avg.} & \textbf{0.63} & \textbf{0.53} & \textbf{0.75} \\
% % \cmidrule(l){1-5}
% Prompt Engineering   
%     & low     & 0.46 (0.18) & 1.58  & 0.73 (0.10) \\
%     & medium  & 0.59 (0.18) & 0.00  & 0.74 (0.11) \\
%     & high    & 0.53 (0.13) & 0.00  & 0.74 (0.10) \\
%     & \textbf{Avg.} & \textbf{0.53} & \textbf{0.53} & \textbf{0.74} \\
% % \cmidrule(l){1-5}
% RAG         
%     & low     & 0.58 (0.17) & 2.38  & 0.74 (0.07) \\
%     & medium  & 0.64 (0.16) & 3.38  & 0.75 (0.04) \\
%     & high    & 0.63 (0.14) & 0.00  & 0.73 (0.08) \\
%     & \textbf{Avg.} & \textbf{0.62} & \textbf{0.00} & \textbf{0.74} \\
% % \cmidrule(l){1-5}
% \textbf{\textit{Controlled-Literacy}}
% % Controlled-Literacy  
%     & low     & 0.79 (0.16) & 0.00  & 0.75 (0.04) \\
%     & medium  & 0.62 (0.13) & 0.00  & 0.75 (0.04) \\
%     & high    & 0.88 (0.18) & 0.00  & 0.74 (0.05) \\
%     & \cellcolor{gray!20}\textbf{Avg.} & \cellcolor{gray!20}\textbf{0.76} & \cellcolor{gray!20}\textbf{0.00} & \cellcolor{gray!20}\textbf{0.75} \\

\bottomrule
\end{tabular}
\caption{Best cross generalization performance on \textbf{CheckCovid Dataset}. The best overall performance in each category is highlighted in gray. Complete results in Appendix \ref{Appendix: Cross Generalization}.}
\label{tab:checkcovid_results}
\end{table*}


==> latex/table_tex_main/Check_Covid_withfact.tex <==
\begin{table*}[htb!]
\centering
\small
\renewcommand{\arraystretch}{0.7}
\begin{tabular}{llcccc}
\toprule
\textbf{Method} & \textbf{Literacy Level} & \textbf{Politeness} & \textbf{Target Distance (↓)} & \textbf{User Preference} & \textbf{Factual Accuracy}\\
\midrule

\multicolumn{5}{l}{\textbf{LLaMA-8B}} \\
% Direct Prompt        
%     & low     & 0.53 (0.22) & 11.98 & 0.63 (0.25) \\
%     & medium  & 0.70 (0.18) & 13.44 & 0.72 (0.09) \\
%     & high    & 0.54 (0.15) & 0.00  & 0.74 (0.05) \\
%     & \textbf{Avg.} & \textbf{0.59} & \textbf{8.47} & \textbf{0.70} \\
% \cmidrule(l){1-5}

Instructional Prompt  
    & low     & 0.52 (0.19) & 0.00  & 0.74 (0.06) &0.87\\
    & medium  & 0.60 (0.17) & 0.21  & 0.74 (0.08) &0.86\\
    & high    & 0.51 (0.12) & 0.00  & 0.74 (0.07) &0.76\\
    & \textbf{Avg.} & \textbf{0.54} & \textbf{0.07} & \textbf{0.74} & \textbf{0.83}\\
% \cmidrule(l){1-5}

RAG       
    & low     & 0.72 (0.19) & 0.00  & 0.74 (0.06) &0.82\\
    & medium  & 0.74 (0.16) & 0.00  & 0.74 (0.07) &0.85\\
    & high    & 0.57 (0.13) & 0.00  & 0.70 (0.11) &0.88\\
    & \textbf{Avg.} & \textbf{0.68} & \textbf{0.00} & \textbf{0.73} &\textbf{0.85}\\
% \cmidrule(l){1-5}
\textbf{\textit{Controlled-Literacy}}

% Controlled-Literacy 
    & low     & 0.82 (0.12) & 0.00  & 0.75 (0.00) &0.92\\
    & medium  & 0.75 (0.15) & 0.00  & 0.75 (0.02) &0.91\\
    & high    & 0.99 (0.00) & 0.00  & 0.75 (0.02) &0.96\\
    & \cellcolor{gray!20}\textbf{Avg.} & \cellcolor{gray!20}\textbf{0.85} & \cellcolor{gray!20}\textbf{0.00} & \cellcolor{gray!20}\textbf{0.75}& \cellcolor{gray!20}\textbf{0.93}\\

\midrule
\multicolumn{5}{l}{\textbf{LLaMA-1B}} \\
% Direct Prompt       
%     & low     & 0.59 (0.27) & 15.32 & 0.52 (0.24) \\
%     & medium  & 0.67 (0.22) & 8.36  & 0.51 (0.20) \\
%     & high    & 0.52 (0.21) & 0.00  & 0.62 (0.17) \\
%     & \textbf{Avg.} & \textbf{0.59} & \textbf{7.89} & \textbf{0.55} \\
% \cmidrule(l){1-5}

Instructional Prompt   
    & low     & 0.68 (0.21) & 1.43  & 0.65 (0.19) &0.57\\
    & medium  & 0.50 (0.19) & 16.56 & 0.55 (0.23) &0.59\\
    & high    & 0.84 (0.17) & 0.00  & 0.65 (0.16) &0.46\\
    & \textbf{Avg.} & \textbf{0.67} & \textbf{6.00} & \textbf{0.62} &\textbf{0.54}\\
% \cmidrule(l){1-5}

RAG         
    & low     & 0.52 (0.19) & 15.93 & 0.41 (0.24) &0.69\\
    & medium  & 0.55 (0.15) & 5.37  & 0.43 (0.23) &0.59\\
    & high    & 0.57 (0.17) & 0.00  & 0.43 (0.21) &0.51\\
    & \textbf{Avg.} & \textbf{0.55} & \textbf{7.10} & \textbf{0.42} &\textbf{0.60}\\
% \cmidrule(l){1-5}



\textbf{\textit{Controlled-Literacy}}
% Controlled-Literacy 
    & low     & 0.80 (0.14) & 0.00  & 0.71 (0.13) &0.69\\
    & medium  & 0.79 (0.17) & 0.00  & 0.72 (0.10) &0.74\\
    & high    & 0.83 (0.27) & 0.00  & 0.68 (0.13) &0.75\\
    & \cellcolor{gray!20}\textbf{Avg.} & \cellcolor{gray!20}\textbf{0.81} & \cellcolor{gray!20}\textbf{0.00} & \cellcolor{gray!20}\textbf{0.70} &\cellcolor{gray!20}\textbf{0.73}\\

\midrule
\multicolumn{5}{l}{\textbf{Qwen-7B}} \\
% Direct Prompt       
%     & low     & 0.74 (0.24) & 0.00  & 0.76 (0.08) \\
%     & medium  & 0.64 (0.21) & 1.58  & 0.75 (0.04) \\
%     & high    & 0.52 (0.15) & 0.00  & 0.75 (0.01) \\
%     & \textbf{Avg.} & \textbf{0.63} & \textbf{0.53} & \textbf{0.75} \\
% \cmidrule(l){1-5}





Instructional Prompt  
    & low     & 0.46 (0.18) & 1.58  & 0.73 (0.10) &0.84\\
    & medium  & 0.59 (0.18) & 0.00  & 0.74 (0.11) &0.95\\
    & high    & 0.53 (0.13) & 0.00  & 0.74 (0.10) &0.97\\
    & \textbf{Avg.} & \textbf{0.53} & \textbf{0.53} & \textbf{0.74} &\textbf{0.92}\\
% \cmidrule(l){1-5}
RAG         
    & low     & 0.58 (0.17) & 2.38  & 0.74 (0.07) &0.88\\
    & medium  & 0.64 (0.16) & 3.38  & 0.75 (0.04) &0.95\\
    & high    & 0.63 (0.14) & 0.00  & 0.73 (0.08) &0.92\\
    & \textbf{Avg.} & \textbf{0.62} & \textbf{0.00} & \textbf{0.74} &\textbf{0.92}\\
% \cmidrule(l){1-5}
\textbf{\textit{Controlled-Literacy}}
% Controlled-Literacy  
    & low     & 0.79 (0.16) & 0.00  & 0.75 (0.04) &0.90\\
    & medium  & 0.62 (0.13) & 0.00  & 0.75 (0.04) &0.97\\
    & high    & 0.88 (0.18) & 0.00  & 0.74 (0.05) &0.98\\
    & \cellcolor{gray!20}\textbf{Avg.} & \cellcolor{gray!20}\textbf{0.76} & \cellcolor{gray!20}\textbf{0.00} & \cellcolor{gray!20}\textbf{0.75} &\cellcolor{gray!20}\textbf{0.95}\\

\bottomrule
\end{tabular}
\caption{Cross generalization performance on \textbf{CheckCovid Dataset}. The best overall performance in each category is highlighted in gray.}
\label{tab:checkcovid_results}
\end{table*}


==> latex/table_tex_main/MisInfo.tex <==
\begin{table*}[htb!]
\centering
\small
\renewcommand{\arraystretch}{0.9}
\begin{tabular}{llccc}
\toprule
\textbf{Method} & \textbf{Literacy Level} & \textbf{Politeness} & \textbf{Target Distance (↓)} & \textbf{User Preference} \\
\midrule
\multicolumn{5}{l}{\textbf{LLaMA-8B}} \\
Direct Prompt        & low     & 0.45 (0.21) & 11.81 & 0.74 (0.10) \\
                     & medium  & 0.57 (0.24) & 8.55  & 0.75 (0.00) \\
                     & high    & 0.24 (0.18) & 0.00  & 0.75 (0.00) \\
\textbf{}            & \textbf{Avg.} & \textbf{0.42} & \textbf{6.79} & \textbf{0.75} \\
Prompt Engineering   & low     & 0.41 (0.24) & 0.00  & 0.75 (0.02) \\
                     & medium  & 0.42 (0.20) & 0.00  & 0.75 (0.01) \\
                     & high    & 0.29 (0.17) & 0.00  & 0.75 (0.04) \\
\textbf{}            & \textbf{Avg.} & \textbf{0.37} & \textbf{0.00} & \textbf{0.75} \\
RAG                  & low     & 0.86 (0.15) & 0.00  & 0.75 (0.00) \\
                     & medium  & 0.72 (0.24) & 0.00  & 0.75 (0.03) \\
                     & high    & 0.34 (0.18) & 0.00  & 0.74 (0.04) \\
\textbf{}            & \textbf{Avg.} & \textbf{0.64} & \textbf{0.00} & \textbf{0.75} \\
\textbf{\textit{Controlled-Literacy}} & low     & 0.92 (0.09) & 0.00  & 0.75 (0.00) \\
                     & medium  & 0.68 (0.23) & 0.00  & 0.75 (0.00) \\
                     & high    & 0.97 (0.02) & 0.00  & 0.75 (0.00) \\
\textbf{}            & \cellcolor{gray!20}\textbf{Avg.} & \cellcolor{gray!20}\textbf{0.86} & \cellcolor{gray!20}\textbf{0.00} & \cellcolor{gray!20}\textbf{0.75} \\
\midrule
\multicolumn{5}{l}{\textbf{LLaMA-1B}} \\
Direct Prompt        & low     & 0.47 (0.32) & 13.94 & 0.57 (0.22) \\
                     & medium  & 0.57 (0.29) & 8.18  & 0.59 (0.21) \\
                     & high    & 0.41 (0.27) & 0.00  & 0.69 (0.13) \\
\textbf{}            & \textbf{Avg.} & \textbf{0.48} & \textbf{7.37} & \textbf{0.62} \\
Prompt Engineering   & low     & 0.73 (0.28) & 10.83 & 0.64 (0.18) \\
                     & medium  & 0.47 (0.32) & 14.06 & 0.59 (0.22) \\
                     & high    & 0.82 (0.18) & 0.00  & 0.68 (0.15) \\
\textbf{}            & \textbf{Avg.} & \textbf{0.67} & \textbf{8.30} & \textbf{0.64} \\
RAG                  & low     & 0.43 (0.30) & 15.05 & 0.53 (0.23) \\
                     & medium  & 0.36 (0.25) & 0.00  & 0.48 (0.23) \\
                     & high    & 0.33 (0.23) & 0.00  & 0.49 (0.21) \\
\textbf{}            & \textbf{Avg.} & \textbf{0.37} & \textbf{5.02} & \textbf{0.41} \\
\textbf{\textit{Controlled-Literacy}} & low     & 0.84 (0.16) & 1.31  & 0.68 (0.17) \\
                     & medium  & 0.61 (0.23) & 3.25  & 0.72 (0.08) \\
                     & high    & 0.92 (0.20) & 0.00  & 0.68 (0.13) \\
\textbf{}            & \cellcolor{gray!20}\textbf{Avg.} & \cellcolor{gray!20}\textbf{0.79} & \cellcolor{gray!20}\textbf{1.52} & \cellcolor{gray!20}\textbf{0.69} \\
\midrule
\multicolumn{5}{l}{\textbf{Qwen-7B}} \\
Direct Prompt        & low     & 0.61 (0.26) & 2.48  & 0.76 (0.06) \\
                     & medium  & 0.66 (0.29) & 2.46  & 0.75 (0.03) \\
                     & high    & 0.36 (0.21) & 0.00  & 0.75 (0.00) \\
\textbf{}            & \textbf{Avg.} & \textbf{0.54} & \textbf{1.65} & \textbf{0.75} \\
Prompt Engineering   & low     & 0.31 (0.22) & 0.00  & 0.74 (0.06) \\
                     & medium  & 0.45 (0.23) & 0.00  & 0.74 (0.10) \\
                     & high    & 0.38 (0.21) & 0.00  & 0.74 (0.05) \\
\textbf{}            & \textbf{Avg.} & \textbf{0.38} & \textbf{0.00} & \textbf{0.74} \\
RAG                  & low     & 0.59 (0.22) & 1.22  & 0.75 (0.01) \\
                     & medium  & 0.52 (0.22) & 0.00  & 0.75 (0.03) \\
                     & high    & 0.49 (0.26) & 0.00  & 0.74 (0.04) \\
\textbf{}            & \textbf{Avg.} & \textbf{0.53} & \textbf{0.41} & \textbf{0.75} \\
\textbf{\textit{Controlled-Literacy}} & low     & 0.78 (0.19) & 0.60  & 0.75 (0.00) \\
                     & medium  & 0.43 (0.16) & 0.00  & 0.75 (0.03) \\
                     & high    & 0.77 (0.30) & 0.00  & 0.75 (0.00) \\
\textbf{}            & \cellcolor{gray!20}\textbf{Avg.} & \cellcolor{gray!20}\textbf{0.66} & \cellcolor{gray!20}\textbf{0.20} & \cellcolor{gray!20}\textbf{0.75} \\
\bottomrule
\end{tabular}
\caption{Cross generalization performance on \textbf{MisinfoCorrect  Dataset}. The best overall performance in each category is highlighted in gray.}
\label{tab:misinfo_correct_results}
\end{table*}


==> latex/table_tex_main/MisInfo_best.tex <==
\begin{table*}[htb!]
\centering
\small
\renewcommand{\arraystretch}{0.9}
\begin{tabular}{llccc}
\toprule
\textbf{Method} & \textbf{Literacy Level} & \textbf{Politeness} & \textbf{Target Distance (↓)} & \textbf{User Preference} \\
\midrule
\multicolumn{5}{l}{\textbf{LLaMA-8B}} \\
Direct Prompt        & low     & 0.45 (0.21) & 11.81 & 0.74 (0.10) \\
                     & medium  & 0.57 (0.24) & 8.55  & 0.75 (0.00) \\
                     & high    & 0.24 (0.18) & 0.00  & 0.75 (0.00) \\
\textbf{}            & \textbf{Avg.} & \textbf{0.42} & \textbf{6.79} & \textbf{0.75} \\
Prompt Engineering   & low     & 0.41 (0.24) & 0.00  & 0.75 (0.02) \\
                     & medium  & 0.42 (0.20) & 0.00  & 0.75 (0.01) \\
                     & high    & 0.29 (0.17) & 0.00  & 0.75 (0.04) \\
\textbf{}            & \textbf{Avg.} & \textbf{0.37} & \textbf{0.00} & \textbf{0.75} \\
RAG                  & low     & 0.86 (0.15) & 0.00  & 0.75 (0.00) \\
                     & medium  & 0.72 (0.24) & 0.00  & 0.75 (0.03) \\
                     & high    & 0.34 (0.18) & 0.00  & 0.74 (0.04) \\
\textbf{}            & \textbf{Avg.} & \textbf{0.64} & \textbf{0.00} & \textbf{0.75} \\
\textbf{\textit{Controlled-Literacy}} & low     & 0.92 (0.09) & 0.00  & 0.75 (0.00) \\
                     & medium  & 0.68 (0.23) & 0.00  & 0.75 (0.00) \\
                     & high    & 0.97 (0.02) & 0.00  & 0.75 (0.00) \\
\textbf{}            & \cellcolor{gray!20}\textbf{Avg.} & \cellcolor{gray!20}\textbf{0.86} & \cellcolor{gray!20}\textbf{0.00} & \cellcolor{gray!20}\textbf{0.75} \\
% \midrule
% \multicolumn{5}{l}{\textbf{LLaMA-1B}} \\
% Direct Prompt        & low     & 0.47 (0.32) & 13.94 & 0.57 (0.22) \\
%                      & medium  & 0.57 (0.29) & 8.18  & 0.59 (0.21) \\
%                      & high    & 0.41 (0.27) & 0.00  & 0.69 (0.13) \\
% \textbf{}            & \textbf{Avg.} & \textbf{0.48} & \textbf{7.37} & \textbf{0.62} \\
% Prompt Engineering   & low     & 0.73 (0.28) & 10.83 & 0.64 (0.18) \\
%                      & medium  & 0.47 (0.32) & 14.06 & 0.59 (0.22) \\
%                      & high    & 0.82 (0.18) & 0.00  & 0.68 (0.15) \\
% \textbf{}            & \textbf{Avg.} & \textbf{0.67} & \textbf{8.30} & \textbf{0.64} \\
% RAG                  & low     & 0.43 (0.30) & 15.05 & 0.53 (0.23) \\
%                      & medium  & 0.36 (0.25) & 0.00  & 0.48 (0.23) \\
%                      & high    & 0.33 (0.23) & 0.00  & 0.49 (0.21) \\
% \textbf{}            & \textbf{Avg.} & \textbf{0.37} & \textbf{5.02} & \textbf{0.41} \\
% \textbf{\textit{Controlled-Literacy}} & low     & 0.84 (0.16) & 1.31  & 0.68 (0.17) \\
%                      & medium  & 0.61 (0.23) & 3.25  & 0.72 (0.08) \\
%                      & high    & 0.92 (0.20) & 0.00  & 0.68 (0.13) \\
% \textbf{}            & \cellcolor{gray!20}\textbf{Avg.} & \cellcolor{gray!20}\textbf{0.79} & \cellcolor{gray!20}\textbf{1.52} & \cellcolor{gray!20}\textbf{0.69} \\
% \midrule
% \multicolumn{5}{l}{\textbf{Qwen-7B}} \\
% Direct Prompt        & low     & 0.61 (0.26) & 2.48  & 0.76 (0.06) \\
%                      & medium  & 0.66 (0.29) & 2.46  & 0.75 (0.03) \\
%                      & high    & 0.36 (0.21) & 0.00  & 0.75 (0.00) \\
% \textbf{}            & \textbf{Avg.} & \textbf{0.54} & \textbf{1.65} & \textbf{0.75} \\
% Prompt Engineering   & low     & 0.31 (0.22) & 0.00  & 0.74 (0.06) \\
%                      & medium  & 0.45 (0.23) & 0.00  & 0.74 (0.10) \\
%                      & high    & 0.38 (0.21) & 0.00  & 0.74 (0.05) \\
% \textbf{}            & \textbf{Avg.} & \textbf{0.38} & \textbf{0.00} & \textbf{0.74} \\
% RAG                  & low     & 0.59 (0.22) & 1.22  & 0.75 (0.01) \\
%                      & medium  & 0.52 (0.22) & 0.00  & 0.75 (0.03) \\
%                      & high    & 0.49 (0.26) & 0.00  & 0.74 (0.04) \\
% \textbf{}            & \textbf{Avg.} & \textbf{0.53} & \textbf{0.41} & \textbf{0.75} \\
% \textbf{\textit{Controlled-Literacy}} & low     & 0.78 (0.19) & 0.60  & 0.75 (0.00) \\
%                      & medium  & 0.43 (0.16) & 0.00  & 0.75 (0.03) \\
%                      & high    & 0.77 (0.30) & 0.00  & 0.75 (0.00) \\
% \textbf{}            & \cellcolor{gray!20}\textbf{Avg.} & \cellcolor{gray!20}\textbf{0.66} & \cellcolor{gray!20}\textbf{0.20} & \cellcolor{gray!20}\textbf{0.75} \\
\bottomrule
\end{tabular}
\caption{Best cross generalization performance on \textbf{MisinfoCorrect  Dataset}. The best overall performance in each category is highlighted in gray. Complete results in Appendix \ref{Appendix: Cross Generalization}.}
\label{tab:misinfo_correct_results}
\end{table*}


==> latex/table_tex_main/MisInfo_withfact.tex <==
\begin{table*}[htb!]
\centering
\small
\renewcommand{\arraystretch}{0.7}
\begin{tabular}{llccccc}
\toprule
\textbf{Method} & \textbf{Literacy Level} & \textbf{Politeness} & \textbf{Target Distance (↓)} & \textbf{User Preference}& \textbf{Factual Accuracy} \\
\midrule
\multicolumn{5}{l}{\textbf{LLaMA-8B}} \\
% Direct Prompt        & low     & 0.45 (0.21) & 11.81 & 0.74 (0.10) \\
%                      & medium  & 0.57 (0.24) & 8.55  & 0.75 (0.00) \\
%                      & high    & 0.24 (0.18) & 0.00  & 0.75 (0.00) \\
% \textbf{}            & \textbf{Avg.} & \textbf{0.42} & \textbf{6.79} & \textbf{0.75} \\

% \textbf{0.98}
Instructional Prompt    
& low     & 0.41 (0.24) & 0.00  & 0.75 (0.02) &0.98\\
& medium  & 0.42 (0.20) & 0.00  & 0.75 (0.01) &0.98\\
& high    & 0.29 (0.17) & 0.00  & 0.75 (0.04) &0.99\\
\textbf{}            & \textbf{Avg.} & \textbf{0.37} & \textbf{0.00} & \textbf{0.75} & \textbf{0.98}\\
RAG              

& low     & 0.86 (0.15) & 0.00  & 0.75 (0.00) &0.99\\
& medium  & 0.72 (0.24) & 0.00  & 0.75 (0.03) &1.00\\
& high    & 0.34 (0.18) & 0.00  & 0.74 (0.04) &0.97\\
\textbf{}            & \textbf{Avg.} & \textbf{0.64} & \textbf{0.00} & \textbf{0.75} & \textbf{0.99}\\

\textbf{\textit{Controlled-Literacy}} 
& low     & 0.92 (0.09) & 0.00  & 0.75 (0.00) &1.00\\
& medium  & 0.68 (0.23) & 0.00  & 0.75 (0.00) &1.00\\
& high    & 0.97 (0.02) & 0.00  & 0.75 (0.00) &1.00\\
\textbf{}            & \cellcolor{gray!20}\textbf{Avg.} & \cellcolor{gray!20}\textbf{0.86} & \cellcolor{gray!20}\textbf{0.00} & \cellcolor{gray!20}\textbf{0.75} & \cellcolor{gray!20}\textbf{1.00}\\
\midrule

\multicolumn{5}{l}{\textbf{LLaMA-1B}} \\
% Direct Prompt        & low     & 0.47 (0.32) & 13.94 & 0.57 (0.22) \\
%                      & medium  & 0.57 (0.29) & 8.18  & 0.59 (0.21) \\
%                      & high    & 0.41 (0.27) & 0.00  & 0.69 (0.13) \\
% \textbf{}            & \textbf{Avg.} & \textbf{0.48} & \textbf{7.37} & \textbf{0.62} \\



Instructional Prompt    
& low     & 0.73 (0.28) & 10.83 & 0.64 (0.18) &0.62\\
& medium  & 0.47 (0.32) & 14.06 & 0.59 (0.22) &0.72\\
& high    & 0.82 (0.18) & 0.00  & 0.68 (0.15) &0.78\\
\textbf{}            & \textbf{Avg.} & \textbf{0.67} & \textbf{8.30} & \textbf{0.64} &\textbf{0.71}\\

RAG                  
& low     & 0.43 (0.30) & 15.05 & 0.53 (0.23) &0.68\\
& medium  & 0.36 (0.25) & 0.00  & 0.48 (0.23) &0.79\\
& high    & 0.33 (0.23) & 0.00  & 0.49 (0.21) &0.76\\
\textbf{}            & \textbf{Avg.} & \textbf{0.37} & \textbf{5.02} & \textbf{0.41} &\textbf{0.74}\\

\textbf{\textit{Controlled-Literacy}} 
& low     & 0.84 (0.16) & 1.31  & 0.68 (0.17) &0.74\\
& medium  & 0.61 (0.23) & 3.25  & 0.72 (0.08) &0.70\\
& high    & 0.92 (0.20) & 0.00  & 0.68 (0.13) &0.81\\
\textbf{}            & \cellcolor{gray!20}\textbf{Avg.} & \cellcolor{gray!20}\textbf{0.79} & \cellcolor{gray!20}\textbf{1.52} & \cellcolor{gray!20}\textbf{0.69} & \cellcolor{gray!20}\textbf{0.75}\\
\midrule
\multicolumn{5}{l}{\textbf{Qwen-7B}} \\
% Direct Prompt        & low     & 0.61 (0.26) & 2.48  & 0.76 (0.06) \\
%                      & medium  & 0.66 (0.29) & 2.46  & 0.75 (0.03) \\
%                      & high    & 0.36 (0.21) & 0.00  & 0.75 (0.00) \\

% \textbf{}            & \textbf{Avg.} & \textbf{0.54} & \textbf{1.65} & \textbf{0.75} \\



Instructional Prompt    
& low     & 0.31 (0.22) & 0.00  & 0.74 (0.06) &0.91\\
& medium  & 0.45 (0.23) & 0.00  & 0.74 (0.10) &0.97\\
& high    & 0.38 (0.21) & 0.00  & 0.74 (0.05) &1.00\\
\textbf{}            & \textbf{Avg.} & \textbf{0.38} & \textbf{0.00} & \textbf{0.74} &\textbf{0.96}
\\

RAG                  
& low     & 0.59 (0.22) & 1.22  & 0.75 (0.01) &0.97\\
& medium  & 0.52 (0.22) & 0.00  & 0.75 (0.03) &0.96\\
& high    & 0.49 (0.26) & 0.00  & 0.74 (0.04) &1.00\\
\textbf{}            & \textbf{Avg.} & \textbf{0.53} & \textbf{0.41} & \textbf{0.75} &\textbf{0.98}\\

\textbf{\textit{Controlled-Literacy}} 
& low     & 0.78 (0.19) & 0.60  & 0.75 (0.00) &1.00\\
& medium  & 0.43 (0.16) & 0.00  & 0.75 (0.03) &0.99\\
& high    & 0.77 (0.30) & 0.00  & 0.75 (0.00) &1.00\\
\textbf{}            & \cellcolor{gray!20}\textbf{Avg.} & \cellcolor{gray!20}\textbf{0.66} & \cellcolor{gray!20}\textbf{0.20} & \cellcolor{gray!20}\textbf{0.75} &\cellcolor{gray!20}\textbf{1.00}\\
\bottomrule
\end{tabular}
\caption{Cross generalization performance on \textbf{MisinfoCorrect  Dataset}. The best overall performance in each category is highlighted in gray.}
\label{tab:misinfo_correct_results}
\end{table*}


==> latex/table_tex_main/Topk.tex <==
\begin{table*}[ht]
\centering
\small
\begin{tabular}{llcccc}
% \renewcommand{\arraystretch}{1.4}
\resizebox{0.48\textwidth}{!}{
\toprule
\textbf{Health Literacy Level} & \textbf{\textit{Top-$k$}} & \textbf{Politeness} & \textbf{Target Distance} & \textbf{User Preference} & \textbf{Factual Accuracy} \\
\midrule
\multirow{3}{*}{Low} 
  & top\_10 & 0.72 (0.25) & 0.00 & 0.71 (0.13) & \textbf{0.89} \\
  & top\_5  & \textbf{0.73} (0.25) & 0.00 & 0.71 (0.12) & 0.87 \\
  & top\_3  & 0.71 (0.25) & 0.00 & \textbf{0.73} (0.09) & 0.84 \\
\midrule
\multirow{3}{*}{Medium} 
  & top\_10 & 0.66 (0.22) & 0.00 & 0.71 (0.13) & 0.81 \\
  & top\_5  & 0.70 (0.22) & 0.00 & 0.72 (0.10) & 0.87 \\
  & top\_3  & \textbf{0.71} (0.23) & 0.00 & \textbf{0.73} (0.11) & \textbf{0.88} \\
\midrule
\multirow{3}{*}{High} 
  & top\_10 & 0.41 (0.21) & 0.00 & \textbf{0.72} (0.09) & \textbf{0.90} \\
  & top\_5  & \textbf{0.43 (0.21)} & 0.00 & 0.71 (0.10) & 0.89 \\
  & top\_3  & 0.42 (0.21) & 0.00 & 0.71 (0.10) & 0.81 \\
\bottomrule
\end{tabular}}
\caption{Comparison of \textit{Top-$k$} selections.}
\label{tab:topk_eval}
\end{table*}


==> latex/table_tex_main/main-qwen.tex <==
\begin{table*}[bth!]
\centering
\small
\renewcommand{\arraystretch}{0.9}
\begin{tabular}{llcccc}
\toprule
\textbf{Method} & \textbf{Literacy Level} & \textbf{Politeness} & \textbf{Target Distance (↓)} & \textbf{User Preference} & \textbf{Refutation} \\
\midrule

% \multicolumn{5}{l}{\textbf{LLaMA-8B}} \\
% Direct Prompt 
%     & low    & 0.51 (0.20) & 16.64 & 0.73 (0.12) \\
%     & medium & 0.62 (0.24) & 12.94 & 0.73 (0.07) \\
%     & high   & 0.36 (0.22) & 0.00  & 0.75 (0.03) \\
%     & \textbf{Avg.} & \textbf{0.50} & \textbf{9.86} & \textbf{0.74} \\
% Prompt Engineering 
%     & low    & 0.39 (0.23) & 0.00 & 0.75 (0.03) \\
%     & medium & 0.49 (0.22) & 1.07 & 0.74 (0.06) \\
%     & high   & 0.35 (0.19) & 0.00 & 0.75 (0.04) \\
%     & \textbf{Avg.} & \textbf{0.41} & \textbf{0.36} & \textbf{0.75} \\
% RAG
%     & low    & 0.72 (0.25) & 0.00 & 0.71 (0.13) \\
%     & medium & 0.66 (0.22) & 0.00 & 0.71 (0.13) \\
%     & high   & 0.41 (0.21) & 0.00 & 0.72 (0.09) \\
%     & \textbf{Avg.} & \textbf{0.60} & \textbf{0.00} & \textbf{0.71} \\
% \textbf{\textit{Controlled-Literacy}} 

%     & low    & 0.84 (0.15) & 0.00 & 0.74 (0.07) \\
%     & medium & 0.69 (0.20) & 0.00 & 0.73 (0.10) \\
%     & high   & 0.98 (0.02) & 0.00 & 0.75 (0.00) \\
%     & \cellcolor{gray!20}\textbf{Avg.} & \cellcolor{gray!20}\textbf{0.84} & \cellcolor{gray!20}\textbf{0.00} & \cellcolor{gray!20}\textbf{0.74} \\
% \midrule


\multicolumn{6}{l}{\textbf{Qwen-7B}} \\
Direct Prompt 
    & low    & 0.65 (0.28) & 0.00 & 0.75 (0.05) &0.60 (0.18)\\
    & medium & 0.65 (0.26) & 4.87 & 0.75 (0.02) &0.70 (0.13)\\
    & high   & 0.37 (0.22) & 0.00 & 0.75 (0.00) &0.74 (0.09)\\
    & \textbf{Avg.} & \textbf{0.56} & \textbf{1.62} & \textbf{0.75} &\textbf{0.68}\\
Prompt Engineering 
    & low    & 0.36 (0.22) & 0.00 & 0.74 (0.06) &0.63 (0.16)\\
    & medium & 0.48 (0.23) & 0.00 & 0.73 (0.13) &0.69 (0.16)\\
    & high   & 0.41 (0.18) & 0.00 & 0.73 (0.12) &0.74 (0.16)\\
    & \textbf{Avg.} & \textbf{0.42} & \textbf{0.00} & \textbf{0.73} & \textbf{0.69}\\
RAG 
    & low    & 0.69 (0.25) & 0.00 & 0.69 (0.16) &0.44 (0.26)\\
    & medium & 0.52 (0.18) & 0.00 & 0.68 (0.18) &0.56 (0.27)\\
    & high   & 0.45 (0.19) & 0.00 & 0.73 (0.07) &0.68 (0.15)\\
    & \textbf{Avg.} & \textbf{0.55} & \textbf{0.00} & \textbf{0.70} & \textbf{0.56}\\
\textbf{\textit{Controlled-Literacy}} 
    & low    & 0.77 (0.18) & 0.00 & 0.73 (0.11) &0.60(0.22)\\
    & medium & 0.55 (0.19) & 0.00 & 0.74 (0.08) &0.64 (0.21)\\
    & high   & 0.86 (0.22) & 0.00 & 0.75 (0.04) &0.68 (0.15)\\
    & \cellcolor{gray!20}\textbf{Avg.} & \cellcolor{gray!20}\textbf{0.73} & \cellcolor{gray!20}\textbf{0.00} & \cellcolor{gray!20}\textbf{0.74} &\cellcolor{gray!20}\textbf{0.64}\\
% \midrule

% \multicolumn{5}{l}{\textbf{LLaMA-1B}} \\
% Direct Prompt 
%     & low     & 0.48 (0.30) & 16.00 & 0.56 (0.21) \\
%     & medium  & 0.52 (0.30) & 8.90  & 0.56 (0.22) \\
%     & high    & 0.34 (0.25) & 0.00  & 0.63 (0.17) \\
%     & \textbf{Avg.} & \textbf{0.45} & \textbf{8.30} & \textbf{0.58} \\
% Prompt Engineering 
%     & low     & 0.65 (0.28) & 6.59  & 0.66 (0.17) \\
%     & medium  & 0.40 (0.25) & 15.93 & 0.58 (0.22) \\
%     & high    & 0.70 (0.24) & 0.00  & 0.68 (0.14) \\
%     & \textbf{Avg.} & \textbf{0.58} & \textbf{7.51} & \textbf{0.64} \\
% RAG 
%     & low     & 0.50 (0.31) & 15.18 & 0.45 (0.25) \\
%     & medium  & 0.41 (0.21) & 4.42  & 0.36 (0.25) \\
%     & high    & 0.42 (0.22) & 0.00  & 0.42 (0.22) \\
%     & \textbf{Avg.} & \textbf{0.44} & \textbf{6.53} & \textbf{0.34} \\
% \textbf{\textit{Controlled-Literacy}} 
%     & low     & 0.73 (0.17) & 0.00  & 0.68 (0.15) \\
%     & medium  & 0.63 (0.21) & 0.00  & 0.71 (0.12) \\
%     & high    & 0.85 (0.27) & 0.00  & 0.67 (0.13) \\
%     & \cellcolor{gray!20}\textbf{Avg.} & \cellcolor{gray!20}\textbf{0.74} & \cellcolor{gray!20}\textbf{0.00} & \cellcolor{gray!20}\textbf{0.69} \\
\bottomrule
\end{tabular}
\caption{Counterspeech generation results on \textbf{MisinfoLiteracy Dataset} using Qwen2.5-
7B-Instruct. The best overall performance in each category is highlighted in gray.}
\label{tab:Main_results}
\end{table*}


==> latex/table_tex_main/main_1B.tex <==
\begin{table*}[bth!]
\centering
\small
\renewcommand{\arraystretch}{0.9}
\begin{tabular}{llcccc}
\toprule
\textbf{Method} & \textbf{Literacy Level} & \textbf{Politeness} & \textbf{Target Distance (↓)} & \textbf{User Preference} & \textbf{Refutation}\\
\midrule

% \multicolumn{5}{l}{\textbf{LLaMA-8B}} \\
% Direct Prompt 
%     & low    & 0.51 (0.20) & 16.64 & 0.73 (0.12) \\
%     & medium & 0.62 (0.24) & 12.94 & 0.73 (0.07) \\
%     & high   & 0.36 (0.22) & 0.00  & 0.75 (0.03) \\
%     & \textbf{Avg.} & \textbf{0.50} & \textbf{9.86} & \textbf{0.74} \\
% Prompt Engineering 
%     & low    & 0.39 (0.23) & 0.00 & 0.75 (0.03) \\
%     & medium & 0.49 (0.22) & 1.07 & 0.74 (0.06) \\
%     & high   & 0.35 (0.19) & 0.00 & 0.75 (0.04) \\
%     & \textbf{Avg.} & \textbf{0.41} & \textbf{0.36} & \textbf{0.75} \\
% RAG
%     & low    & 0.72 (0.25) & 0.00 & 0.71 (0.13) \\
%     & medium & 0.66 (0.22) & 0.00 & 0.71 (0.13) \\
%     & high   & 0.41 (0.21) & 0.00 & 0.72 (0.09) \\
%     & \textbf{Avg.} & \textbf{0.60} & \textbf{0.00} & \textbf{0.71} \\
% \textbf{\textit{Controlled-Literacy}} 

%     & low    & 0.84 (0.15) & 0.00 & 0.74 (0.07) \\
%     & medium & 0.69 (0.20) & 0.00 & 0.73 (0.10) \\
%     & high   & 0.98 (0.02) & 0.00 & 0.75 (0.00) \\
%     & \cellcolor{gray!20}\textbf{Avg.} & \cellcolor{gray!20}\textbf{0.84} & \cellcolor{gray!20}\textbf{0.00} & \cellcolor{gray!20}\textbf{0.74} \\
% \midrule

% \multicolumn{5}{l}{\textbf{Qwen-7B}} \\
% Direct Prompt 
%     & low    & 0.65 (0.28) & 0.00 & 0.75 (0.05) \\
%     & medium & 0.65 (0.26) & 4.87 & 0.75 (0.02) \\
%     & high   & 0.37 (0.22) & 0.00 & 0.75 (0.00) \\
%     & \textbf{Avg.} & \textbf{0.56} & \textbf{1.62} & \textbf{0.75} \\
% Prompt Engineering 
%     & low    & 0.36 (0.22) & 0.00 & 0.74 (0.06) \\
%     & medium & 0.48 (0.23) & 0.00 & 0.73 (0.13) \\
%     & high   & 0.41 (0.18) & 0.00 & 0.73 (0.12) \\
%     & \textbf{Avg.} & \textbf{0.42} & \textbf{0.00} & \textbf{0.73} \\
% RAG 
%     & low    & 0.69 (0.25) & 0.00 & 0.69 (0.16) \\
%     & medium & 0.52 (0.18) & 0.00 & 0.68 (0.18) \\
%     & high   & 0.45 (0.19) & 0.00 & 0.73 (0.07) \\
%     & \textbf{Avg.} & \textbf{0.55} & \textbf{0.00} & \textbf{0.70} \\
% \textbf{\textit{Controlled-Literacy}} 
%     & low    & 0.77 (0.18) & 0.00 & 0.73 (0.11) \\
%     & medium & 0.55 (0.19) & 0.00 & 0.74 (0.08) \\
%     & high   & 0.86 (0.22) & 0.00 & 0.75 (0.04) \\
%     & \cellcolor{gray!20}\textbf{Avg.} & \cellcolor{gray!20}\textbf{0.73} & \cellcolor{gray!20}\textbf{0.00} & \cellcolor{gray!20}\textbf{0.74} \\
% \midrule


\multicolumn{6}{l}{\textbf{LLaMA-1B}} \\
Direct Prompt 
    & low     & 0.48 (0.30) & 16.00 & 0.56 (0.21) &0.51 (0.24)\\
    & medium  & 0.52 (0.30) & 8.90  & 0.56 (0.22) &0.60 (0.23)\\
    & high    & 0.34 (0.25) & 0.00  & 0.63 (0.17) &0.67 (0.17)\\
    & \textbf{Avg.} & \textbf{0.45} & \textbf{8.30} & \textbf{0.58} & \textbf{0.59}\\
Prompt Engineering 
    & low     & 0.65 (0.28) & 6.59  & 0.66 (0.17) &0.57 (0.20)\\
    & medium  & 0.40 (0.25) & 15.93 & 0.58 (0.22) &0.64 (0.26)\\
    & high    & 0.70 (0.24) & 0.00  & 0.68 (0.14) &0.69 (0.14)\\
    & \textbf{Avg.} & \textbf{0.58} & \textbf{7.51} & \textbf{0.64} & \textbf{0.63}\\
RAG 
    & low     & 0.50 (0.31) & 15.18 & 0.45 (0.25) &0.38 (0.29)\\
    & medium  & 0.41 (0.21) & 4.42  & 0.36 (0.25) &0.33 (0.30)\\
    & high    & 0.42 (0.22) & 0.00  & 0.42 (0.22) &0.45 (0.28)\\
    & \textbf{Avg.} & \textbf{0.44} & \textbf{6.53} & \textbf{0.34} & \textbf{0.39}\\
\textbf{\textit{Controlled-Literacy}} 
    & low     & 0.73 (0.17) & 0.00  & 0.68 (0.15) &0.52 (0.20)\\
    & medium  & 0.63 (0.21) & 0.00  & 0.71 (0.12) &0.63 (0.18)\\
    & high    & 0.85 (0.27) & 0.00  & 0.67 (0.13) &0.68 (0.13)\\
    & \cellcolor{gray!20}\textbf{Avg.} & \cellcolor{gray!20}\textbf{0.74} & \cellcolor{gray!20}\textbf{0.00} & \cellcolor{gray!20}\textbf{0.69} &\cellcolor{gray!20}\textbf{0.61}\\
\bottomrule
\end{tabular}
\caption{Counterspeech generation results on \textbf{MisinfoLiteracy Dataset} using LLaMA3.2-1B-Instruct. The best overall performance in each category is highlighted in gray.}
\label{tab:Main_results}
\end{table*}


==> latex/table_tex_main/main_8B.tex <==
\begin{table*}[bth!]
\centering
\small
\renewcommand{\arraystretch}{0.5}
\begin{tabular}{llccccc}
\toprule
\textbf{Method} & \textbf{Literacy Level} & \textbf{Politeness} & \textbf{Target Distance (↓)} & \textbf{User Preference} & \textbf{Refutation} & \textbf{Factual Accuracy} \\
\midrule
\multicolumn{7}{l}{\textbf{LLaMA-8B}} \\
Direct Prompt 
    & low    & 0.51 (0.20) & 16.64 & 0.73 (0.12) &0.66 (0.19) &0.81 (0.31)\\
    & medium & 0.62 (0.24) & 12.94 & 0.73 (0.07) &0.72 (0.11) &0.88 (0.21)\\
    & high   & 0.36 (0.22) & 0.00  & 0.75 (0.03) &0.75 (0.09) &0.87 (0.16)\\
    & \textbf{Avg.} & \textbf{0.50} & \textbf{9.86} & \textbf{0.74} & \textbf{0.71} & \textbf{0.85}\\
Prompt Engineering 
    & low    & 0.39 (0.23) & 0.00 & 0.75 (0.03) &0.73 (0.08) &0.84 (0.22) \\
    & medium & 0.49 (0.22) & 1.07 & 0.74 (0.06) &0.73 (0.08) &0.90 (0.20) \\
    & high   & 0.35 (0.19) & 0.00 & 0.75 (0.04) &0.77 (0.08) &0.89 (0.17)\\
    & \textbf{Avg.} & \textbf{0.41} & \textbf{0.36} & \textbf{0.75} & \textbf{0.75} &\textbf{0.88}\\
RAG
    & low    &0.71 (0.25) & 0.00 & 0.71 (0.13)  & 0.55 (0.23) &0.76 (0.27)\\
    & medium & 0.71 (0.23) & 0.00 & 0.73 (0.11) & 0.65 (0.21) &0.84 (0.24)\\
    & high   & 0.41 (0.21) & 0.00 & 0.72 (0.09) & 0.71 (0.13) &0.82 (0.23)\\
    & \textbf{Avg.} & \textbf{0.61} & \textbf{0.00} & \textbf{0.72}& \textbf{0.64} & \textbf{0.81}\\
\textbf{\textit{Controlled-Literacy}} 

    & low    & 0.84 (0.15) & 0.00 & 0.74 (0.07) &0.63 (0.18) &0.80 (0.24)\\
    & medium & 0.69 (0.20) & 0.00 & 0.73 (0.10) &0.70(0.30) &0.75 (0.33)\\
    & high   & 0.98 (0.02) & 0.00 & 0.75 (0.00) &0.73 (0.06) &0.84 (0.15)\\
    & \cellcolor{gray!20}\textbf{Avg.} & \cellcolor{gray!20}\textbf{0.84} & \cellcolor{gray!20}\textbf{0.00} & \cellcolor{gray!20}\textbf{0.74} &\cellcolor{gray!20}\textbf{0.69}  &\cellcolor{gray!20}\textbf{0.80}\\
% \midrule

% \multicolumn{5}{l}{\textbf{Qwen-7B}} \\
% Direct Prompt 
%     & low    & 0.65 (0.28) & 0.00 & 0.75 (0.05) \\
%     & medium & 0.65 (0.26) & 4.87 & 0.75 (0.02) \\
%     & high   & 0.37 (0.22) & 0.00 & 0.75 (0.00) \\
%     & \textbf{Avg.} & \textbf{0.56} & \textbf{1.62} & \textbf{0.75} \\
% Prompt Engineering 
%     & low    & 0.36 (0.22) & 0.00 & 0.74 (0.06) \\
%     & medium & 0.48 (0.23) & 0.00 & 0.73 (0.13) \\
%     & high   & 0.41 (0.18) & 0.00 & 0.73 (0.12) \\
%     & \textbf{Avg.} & \textbf{0.42} & \textbf{0.00} & \textbf{0.73} \\
% RAG 
%     & low    & 0.69 (0.25) & 0.00 & 0.69 (0.16) \\
%     & medium & 0.52 (0.18) & 0.00 & 0.68 (0.18) \\
%     & high   & 0.45 (0.19) & 0.00 & 0.73 (0.07) \\
%     & \textbf{Avg.} & \textbf{0.55} & \textbf{0.00} & \textbf{0.70} \\
% \textbf{\textit{Controlled-Literacy}} 
%     & low    & 0.77 (0.18) & 0.00 & 0.73 (0.11) \\
%     & medium & 0.55 (0.19) & 0.00 & 0.74 (0.08) \\
%     & high   & 0.86 (0.22) & 0.00 & 0.75 (0.04) \\
%     & \cellcolor{gray!20}\textbf{Avg.} & \cellcolor{gray!20}\textbf{0.73} & \cellcolor{gray!20}\textbf{0.00} & \cellcolor{gray!20}\textbf{0.74} \\
% \midrule

% \multicolumn{5}{l}{\textbf{LLaMA-1B}} \\
% Direct Prompt 
%     & low     & 0.48 (0.30) & 16.00 & 0.56 (0.21) \\
%     & medium  & 0.52 (0.30) & 8.90  & 0.56 (0.22) \\
%     & high    & 0.34 (0.25) & 0.00  & 0.63 (0.17) \\
%     & \textbf{Avg.} & \textbf{0.45} & \textbf{8.30} & \textbf{0.58} \\
% Prompt Engineering 
%     & low     & 0.65 (0.28) & 6.59  & 0.66 (0.17) \\
%     & medium  & 0.40 (0.25) & 15.93 & 0.58 (0.22) \\
%     & high    & 0.70 (0.24) & 0.00  & 0.68 (0.14) \\
%     & \textbf{Avg.} & \textbf{0.58} & \textbf{7.51} & \textbf{0.64} \\
% RAG 
%     & low     & 0.50 (0.31) & 15.18 & 0.45 (0.25) \\
%     & medium  & 0.41 (0.21) & 4.42  & 0.36 (0.25) \\
%     & high    & 0.42 (0.22) & 0.00  & 0.42 (0.22) \\
%     & \textbf{Avg.} & \textbf{0.44} & \textbf{6.53} & \textbf{0.34} \\
% \textbf{\textit{Controlled-Literacy}} 
%     & low     & 0.73 (0.17) & 0.00  & 0.68 (0.15) \\
%     & medium  & 0.63 (0.21) & 0.00  & 0.71 (0.12) \\
%     & high    & 0.85 (0.27) & 0.00  & 0.67 (0.13) \\
%     & \cellcolor{gray!20}\textbf{Avg.} & \cellcolor{gray!20}\textbf{0.74} & \cellcolor{gray!20}\textbf{0.00} & \cellcolor{gray!20}\textbf{0.69} \\
\bottomrule
\end{tabular}
\caption{Counterspeech generation results on \textbf{MisinfoLiteracy Dataset} using LLaMA3.1-8B-Instruct categorized by health literacy levels: low, medium, and high, along with the overall average. Higher values for politeness and user preference indicate better performance, while lower values for target distance indicate better alignment. The best overall performance in each category is highlighted in gray.}
\label{tab:Main_results}
\end{table*}


==> latex/table_tex_main/main_results.tex <==
\begin{table*}[bth!]
\centering
\small
\renewcommand{\arraystretch}{0.9}
\begin{tabular}{llccc}
\toprule
\textbf{Method} & \textbf{Literacy Level} & \textbf{Politeness} & \textbf{Target Distance (↓)} & \textbf{User Preference} \\
\midrule

\multicolumn{5}{l}{\textbf{LLaMA-8B}} \\
Direct Prompt 
    & low    & 0.51 (0.20) & 16.64 & 0.73 (0.12) \\
    & medium & 0.62 (0.24) & 12.94 & 0.73 (0.07) \\
    & high   & 0.36 (0.22) & 0.00  & 0.75 (0.03) \\
    & \textbf{Avg.} & \textbf{0.50} & \textbf{9.86} & \textbf{0.74} \\
Prompt Engineering 
    & low    & 0.39 (0.23) & 0.00 & 0.75 (0.03) \\
    & medium & 0.49 (0.22) & 1.07 & 0.74 (0.06) \\
    & high   & 0.35 (0.19) & 0.00 & 0.75 (0.04) \\
    & \textbf{Avg.} & \textbf{0.41} & \textbf{0.36} & \textbf{0.75} \\
RAG
    & low    & 0.72 (0.25) & 0.00 & 0.71 (0.13) \\
    & medium & 0.66 (0.22) & 0.00 & 0.71 (0.13) \\
    & high   & 0.41 (0.21) & 0.00 & 0.72 (0.09) \\
    & \textbf{Avg.} & \textbf{0.60} & \textbf{0.00} & \textbf{0.71} \\
\textbf{\textit{Controlled-Literacy}} 

    & low    & 0.84 (0.15) & 0.00 & 0.74 (0.07) \\
    & medium & 0.69 (0.20) & 0.00 & 0.73 (0.10) \\
    & high   & 0.98 (0.02) & 0.00 & 0.75 (0.00) \\
    & \cellcolor{gray!20}\textbf{Avg.} & \cellcolor{gray!20}\textbf{0.84} & \cellcolor{gray!20}\textbf{0.00} & \cellcolor{gray!20}\textbf{0.74} \\
\midrule

\multicolumn{5}{l}{\textbf{Qwen-7B}} \\
Direct Prompt 
    & low    & 0.65 (0.28) & 0.00 & 0.75 (0.05) \\
    & medium & 0.65 (0.26) & 4.87 & 0.75 (0.02) \\
    & high   & 0.37 (0.22) & 0.00 & 0.75 (0.00) \\
    & \textbf{Avg.} & \textbf{0.56} & \textbf{1.62} & \textbf{0.75} \\
Prompt Engineering 
    & low    & 0.36 (0.22) & 0.00 & 0.74 (0.06) \\
    & medium & 0.48 (0.23) & 0.00 & 0.73 (0.13) \\
    & high   & 0.41 (0.18) & 0.00 & 0.73 (0.12) \\
    & \textbf{Avg.} & \textbf{0.42} & \textbf{0.00} & \textbf{0.73} \\
RAG 
    & low    & 0.69 (0.25) & 0.00 & 0.69 (0.16) \\
    & medium & 0.52 (0.18) & 0.00 & 0.68 (0.18) \\
    & high   & 0.45 (0.19) & 0.00 & 0.73 (0.07) \\
    & \textbf{Avg.} & \textbf{0.55} & \textbf{0.00} & \textbf{0.70} \\
\textbf{\textit{Controlled-Literacy}} 
    & low    & 0.77 (0.18) & 0.00 & 0.73 (0.11) \\
    & medium & 0.55 (0.19) & 0.00 & 0.74 (0.08) \\
    & high   & 0.86 (0.22) & 0.00 & 0.75 (0.04) \\
    & \cellcolor{gray!20}\textbf{Avg.} & \cellcolor{gray!20}\textbf{0.73} & \cellcolor{gray!20}\textbf{0.00} & \cellcolor{gray!20}\textbf{0.74} \\
\midrule

\multicolumn{5}{l}{\textbf{LLaMA-1B}} \\
Direct Prompt 
    & low     & 0.48 (0.30) & 16.00 & 0.56 (0.21) \\
    & medium  & 0.52 (0.30) & 8.90  & 0.56 (0.22) \\
    & high    & 0.34 (0.25) & 0.00  & 0.63 (0.17) \\
    & \textbf{Avg.} & \textbf{0.45} & \textbf{8.30} & \textbf{0.58} \\
Prompt Engineering 
    & low     & 0.65 (0.28) & 6.59  & 0.66 (0.17) \\
    & medium  & 0.40 (0.25) & 15.93 & 0.58 (0.22) \\
    & high    & 0.70 (0.24) & 0.00  & 0.68 (0.14) \\
    & \textbf{Avg.} & \textbf{0.58} & \textbf{7.51} & \textbf{0.64} \\
RAG 
    & low     & 0.50 (0.31) & 15.18 & 0.45 (0.25) \\
    & medium  & 0.41 (0.21) & 4.42  & 0.36 (0.25) \\
    & high    & 0.42 (0.22) & 0.00  & 0.42 (0.22) \\
    & \textbf{Avg.} & \textbf{0.44} & \textbf{6.53} & \textbf{0.34} \\
\textbf{\textit{Controlled-Literacy}} 
    & low     & 0.73 (0.17) & 0.00  & 0.68 (0.15) \\
    & medium  & 0.63 (0.21) & 0.00  & 0.71 (0.12) \\
    & high    & 0.85 (0.27) & 0.00  & 0.67 (0.13) \\
    & \cellcolor{gray!20}\textbf{Avg.} & \cellcolor{gray!20}\textbf{0.74} & \cellcolor{gray!20}\textbf{0.00} & \cellcolor{gray!20}\textbf{0.69} \\
\bottomrule
\end{tabular}
\caption{Counterspeech generation results on \textbf{MisinfoLiteracy Dataset} categorized by health literacy levels: low, medium, and high, along with the overall average. Higher values for politeness and user preference indicate better performance, while lower values for target distance indicate better alignment. The best overall performance in each category is highlighted in gray.}
\label{tab:Main_results}
\end{table*}


==> latex/table_tex_main/main_withfact.tex <==
\begin{table*}[bth!]
\centering
\small
\renewcommand{\arraystretch}{0.7}
\resizebox{0.9\textwidth}{!}{
\begin{tabular}{llcccc}
\toprule
\textbf{Method} & \textbf{Literacy Level} & \textbf{Politeness} & \textbf{Target Distance (↓)} & \textbf{User Preference} & \textbf{Factual Accuracy}\\
\midrule


\multicolumn{5}{l}{\textbf{LLaMA-8B}} \\
% Direct Prompt 
%     & low    & 0.51 (0.20) & 16.64 & 0.73 (0.12) \\
%     & medium & 0.62 (0.24) & 12.94 & 0.73 (0.07) \\
%     & high   & 0.36 (0.22) & 0.00  & 0.75 (0.03) \\
%     & \textbf{Avg.} & \textbf{0.50} & \textbf{9.86} & \textbf{0.74} \\
Instructional Prompt 
    & low    & 0.39 (0.23) & 0.00 & 0.75 (0.03) &0.86\\
    & medium & 0.49 (0.22) & 1.07 & 0.74 (0.06) &0.89\\
    & high   & 0.35 (0.19) & 0.00 & 0.75 (0.04) &0.87\\
    % & \textbf{Avg.} & \textbf{0.41} & \textbf{0.36} & \textbf{0.75}  & \textbf{0.87}\\
    & \textbf{Avg.} & \textbf{0.41} (0.21) & \textbf{0.36} & \textbf{0.75} (0.04)  & \textbf{0.87}\\

RAG
    & low    & 0.72 (0.25) & 0.00 & 0.71 (0.13) &0.89\\
    & medium & 0.66 (0.22) & 0.00 & 0.71 (0.13) &0.88\\
    & high   & 0.41 (0.21) & 0.00 & 0.72 (0.09) &0.90\\
    % & \textbf{Avg.} & \textbf{0.60} & \textbf{0.00} & \textbf{0.71} & \textbf{0.89}\\
    & \textbf{Avg.} & \textbf{0.60} (0.23) & \textbf{0.00} & \textbf{0.71} (0.12) & \textbf{0.89}\\

\textbf{\textit{Controlled-Literacy}} 


    & low    & 0.84 (0.15) & 0.00 & 0.74 (0.07) &0.89\\
    & medium & 0.69 (0.20) & 0.00 & 0.73 (0.10) &0.90\\
    & high   & 0.98 (0.02) & 0.00 & 0.75 (0.00) &0.93\\
    & \cellcolor{gray!20}\textbf{Avg.} & \cellcolor{gray!20}\textbf{0.84} & \cellcolor{gray!20}\textbf{0.00} & \cellcolor{gray!20}\textbf{0.74} &\cellcolor{gray!20}\textbf{0.91}\\
\midrule

\multicolumn{5}{l}{\textbf{Qwen-7B}} \\
% Direct Prompt 
%     & low    & 0.65 (0.28) & 0.00 & 0.75 (0.05) \\
%     & medium & 0.65 (0.26) & 4.87 & 0.75 (0.02) \\
%     & high   & 0.37 (0.22) & 0.00 & 0.75 (0.00) \\
%     & \textbf{Avg.} & \textbf{0.56} & \textbf{1.62} & \textbf{0.75} \\

Instructional Prompt 
    & low    & 0.36 (0.22) & 0.00 & 0.74 (0.06) &0.71\\
    & medium & 0.48 (0.23) & 0.00 & 0.73 (0.13) &0.88\\
    & high   & 0.41 (0.18) & 0.00 & 0.73 (0.12) &0.89\\
    & \textbf{Avg.} & \textbf{0.42} & \textbf{0.00} & \textbf{0.73} &\textbf{0.83}\\
RAG 
    & low    & 0.69 (0.25) & 0.00 & 0.69 (0.16) &0.79\\
    & medium & 0.52 (0.18) & 0.00 & 0.68 (0.18) &0.92\\
    & high   & 0.45 (0.19) & 0.00 & 0.73 (0.07) &0.91\\
    & \textbf{Avg.} & \textbf{0.55} & \textbf{0.00} & \textbf{0.70}  & \textbf{0.87}\\
\textbf{\textit{Controlled-Literacy}} 
    & low    & 0.77 (0.18) & 0.00 & 0.73 (0.11) &0.84\\
    & medium & 0.55 (0.19) & 0.00 & 0.74 (0.08) &0.94\\
    & high   & 0.86 (0.22) & 0.00 & 0.75 (0.04) &0.92\\
    & \cellcolor{gray!20}\textbf{Avg.} & \cellcolor{gray!20}\textbf{0.73} & \cellcolor{gray!20}\textbf{0.00} & \cellcolor{gray!20}\textbf{0.74} &\cellcolor{gray!20}\textbf{0.90}\\
\midrule

\multicolumn{5}{l}{\textbf{LLaMA-1B}} \\
% Direct Prompt 
%     & low     & 0.48 (0.30) & 16.00 & 0.56 (0.21) \\
%     & medium  & 0.52 (0.30) & 8.90  & 0.56 (0.22) \\
%     & high    & 0.34 (0.25) & 0.00  & 0.63 (0.17) \\
%     & \textbf{Avg.} & \textbf{0.45} & \textbf{8.30} & \textbf{0.58} \\

Instructional Prompt
    & low     & 0.65 (0.28) & 6.59  & 0.66 (0.17) &0.50\\
    & medium  & 0.40 (0.25) & 15.93 & 0.58 (0.22) &0.58\\
    & high    & 0.70 (0.24) & 0.00  & 0.68 (0.14)  &0.54\\
    & \textbf{Avg.} & \textbf{0.58} & \textbf{7.51} & \textbf{0.64} &\textbf{0.54}\\
RAG 

    & low     & 0.50 (0.31) & 15.18 & 0.45 (0.25) &0.63\\
    & medium  & 0.41 (0.21) & 4.42  & 0.36 (0.25) &0.71\\
    & high    & 0.42 (0.22) & 0.00  & 0.42 (0.22) &0.63\\
    & \textbf{Avg.} & \textbf{0.44} & \textbf{6.53} & \textbf{0.34}  &\textbf{0.66}\\
\textbf{\textit{Controlled-Literacy}} 


    & low     & 0.73 (0.17) & 0.00  & 0.68 (0.15) &0.61\\
    & medium  & 0.63 (0.21) & 0.00  & 0.71 (0.12) &0.75\\
    & high    & 0.85 (0.27) & 0.00  & 0.67 (0.13) &0.76\\
    & \cellcolor{gray!20}\textbf{Avg.} & \cellcolor{gray!20}\textbf{0.74} & \cellcolor{gray!20}\textbf{0.00} & \cellcolor{gray!20}\textbf{0.69} & \cellcolor{gray!20}\textbf{0.71}\\
\bottomrule
\end{tabular}}
\caption{Counterspeech generation results on \textbf{MisinfoLiteracy} categorized by health literacy levels: low, medium, and high, along with the overall average. User preference only presents the evaluation by intended user category. 
Higher values for politeness, user preference, and factual accuracy indicate better performance, while lower values for target distance indicate better alignment. The best overall performance in each category is highlighted in gray.}
\label{tab:Main_results}
\end{table*}

